Vertex Ordering for Exact Triangle Listing: Concave Geometry and Certified Rounding

Exact forward triangle listers orient each edge of a graph by a vertex order. The order does not change the output, but it changes the work. For the adaptive lister, which scans the smaller of the two forward neighborhoods, the number of candidate tests is a known sum of minima of forward degrees, but how to optimize it had not been characterized. We show that this work is a concave function of the forward degrees, so choosing an order is concave minimization over the orientation polytope, whose vertices are the forward-degree vectors of orders. A single sort therefore rounds any point of the polytope, including the out-degree vector of any orientation, to an order with no more work, with a computable lower bound on the improvement. Minimizing the work is nevertheless NP-hard and APX-hard on triangle-free graphs of maximum degree three, and under the Unique Games Conjecture it has no polynomial-time constant-factor approximation. We also analyze logistic score relaxations and the large-graph limit of degree-based orders; on random cubic graphs, the expected work of every degree-based order is asymptotically at least $2.43$ times the expected optimum. Tangent refinement followed by iterated local search reduces the work by \HeldTIKMean\% on average on nine held-out networks fixed by a pre-registered protocol, and by \NSFrozenTILSMean\% in a supplementary rescoring, specified in advance, against a stronger reference that adds the published Neigh local search. The gains are in candidate tests; we observe no reproducible wall-clock speedup.

==> supp_heldout_rows.tex <==
Email-Eu-core & Neigh3 & 6.51 & 3.22 & 3.17 & 3.26 & 3.50$\pm$0.01 \\
CollegeMsg & Neigh4-rev & 18.82 & 3.04 & 2.86 & 2.75 & 3.07$\pm$0.00 \\
LastFM-Asia & Neigh2 & 2.74 & 5.88 & 4.22 & 4.57 & 6.01$\pm$0.19 \\
Deezer-Europe & Neigh5 & 4.34 & 5.23 & 3.25 & 3.53 & 4.92$\pm$0.02 \\
Amazon0302 & Neigh1-rev & 6.18 & 2.72 & 0.39 & 0.00 & 2.39$\pm$0.05 \\
Wiki-Talk$^\dagger$ & Degree & 0.00 & 13.04 & 11.48 & 10.97 & 13.04$\pm$0.02 \\
com-Youtube & Neigh3-rev & 13.61 & 12.52 & 15.61 & 13.78 & 16.14$\pm$0.01 \\
web-Google & Neigh3-rev & 4.08 & 1.13 & 0.93 & 0.00 & 1.39$\pm$0.00 \\
roadNet-CA & Neigh3-rev & 18.72 & 18.18 & 0.05 & 0.00 & 17.07$\pm$0.00 \\
\midrule
Mean & & 8.33 & 7.22 & 4.66 & 4.32 & 7.50 \\

